A Smooth Lattice construction of the Oppenheimer-Snyder spacetime

We present test results for the smooth lattice method using an Oppenheimer-Snyder spacetime. The results are in excellent agreement with theory and numerical results from other authors.

==> data/crash-test/ah-form-geo.tex <==
% written by programs/geodesic/lattice-evol:evolve
\def\APHformedTimeGeo{10.87837}
\def\APHformedLocationGeo{2.16534}


==> data/crash-test/time-step-geo.tex <==
% written by programs/geodesic/lattice-evol:evolve
\def\TimeStepBegin{5.38\times10^{-3}}


==> data/long-term/ah-form-max.tex <==
% written by programs/maximal/lattice-evol:evolve
\def\APHformedTimeMax{16.98237}
\def\APHformedLocationMax{2.38015}


==> data/long-term/lapse-slope.tex <==
% written by programs/maximal/post-process/least-square
\def\LapseSlope{-0.54455}
\def\LapseSlopeExact{-0.54433}
\def\LapseSlopeBeg{200.0}
\def\LapseSlopeEnd{300.0}

